ViMoTest: A Tool to Specify ViewModel-Based GUI Test Scenarios using Projectional Editing

Automated GUI testing is crucial in ensuring that presentation logic behaves as expected. However, existing tools often apply end-to-end approaches and face challenges such as high specification efforts, maintenance difficulties, and flaky tests while coupling to GUI framework specifics. To address these challenges, we introduce the ViMoTest tool, which leverages Behavior-driven Development, the ViewModel architectural pattern, and projectional Domain-specific Languages (DSLs) to isolate and test presentation logic independently of GUI frameworks. We demonstrate the tool with a small JavaFX-based task manager example and generate executable code.

==> _ICST_25__ViMoTest_Tool_Paper/custom-commands.tex <==
\newcommand{\aspect}[2]{
\noindent
\textbf{#1}: #2
}
\newcommand{\aspectItalic}[2]{
\noindent
\textit{#1}: #2
}

\newcommand{\aspectWithIndent}[2]{
\noindent
\hfill\begin{minipage}{\dimexpr\linewidth-0.4cm}
\textbf{#1}: #2
\end{minipage}
}

\newcommand{\aspectBox}[3]{
\noindent
\fbox{\begin{minipage}{0.96\linewidth}
\textbf{#1} #2: \textit{#3}
\end{minipage}}
}

\newcommand{\simpleBox}[1]{
\noindent
\fbox{\begin{minipage}{0.96\linewidth}
\textit{#1}
\end{minipage}}
}

%%
%% Custom Latex command for formatting problems
\newcommand{\problem}[3]{
\noindent
\textbf{#1} - \textit{#2}: #3
}
%%
%% Custom Latex command for formatting a hypothesis
\newcommand{\hypothesis}[1]{
\vspace{1mm}
\noindent
\textit{Hypothesis}: \textit{#1}
\vspace{1mm}
}

%%
%% Custom Latex command for formatting research questions
\newcommand{\researchquestion}[2]{
\noindent
\fbox{\begin{minipage}{0.96\linewidth}
\textbf{#1:} \textit{#2}
\end{minipage}}
\vspace{2mm}
}

%%
%% Custom Latex command for formatting contributions
\newcommand{\contribution}[3]{
\noindent
\fbox{\begin{minipage}{0.96\linewidth}
\textbf{#1} #2: \textit{#3}
\end{minipage}}
}

\newcommand{\rectIcon}[1]{\includegraphics[height=1.5ex,trim=1mm 3mm 1mm 1mm]{graphics/util/#1.pdf}}
\newcommand{\roundIcon}[1]{\includegraphics[height=1.5ex,trim=1mm 3mm 1mm 1mm]{graphics/util/#1.pdf}}

\newcommand{\numberIcon}[1]{\includegraphics[height=1.5ex,trim=8mm 8mm 8mm 8mm]{graphics/util/#1.pdf}}

